Towards Structured Dynamic Sparse Pre-Training of BERT

Identifying algorithms for computational efficient unsupervised training of large language models is an important and active area of research. In this work, we develop and study a straightforward, dynamic always-sparse pre-training approach for BERT language modeling task, which leverages periodic compression steps based on magnitude pruning followed by random parameter re-allocation. This approach enables us to achieve Pareto improvements in terms of the number of floating-point operations (FLOPs) over statically sparse and dense models across a broad spectrum of network sizes. Furthermore, we demonstrate that training remains FLOP-efficient when using coarse-grained block sparsity, making it particularly promising for efficient execution on modern hardware accelerators.

==> old_version/waste.tex <==
%The algorithms can be largely distinguished according to the frequency of the changes of the sparsity and whether they are compatible with both training and inference time improvements. 
%Many of these algorithms augment the capacity of the representation in order to achieve test time advantages subset of the layers during has been shown to lead to test time advantages~\cite{Fan2019}
%

%Structure introducing regularizers~\cite{Narang2017, Yang2019}
%Extensions of unstructured DynSparse training towards structured sparsity have been previously tested in Ref.~\cite{Mostafa2019} using kernel level sparsity and in a workshop contributions by the authors in Ref.~\cite{Dietrich2021}. Input dependent blocksparsity pattern have been investigated to targeting inference

%Extending gradual pruning pruning and group lasso regularization~\cite{Narang2017}
%Approaches exploiting a low rank representation for pruning have been succesful for downstream task of BERT~\cite{Wang2019d}

%~\cite{Gray2017block}

%An even larger class of sparse training algorithms trains densely and therefore is only able to structured pruning of layers~\cite{Fan2019}, the removal of heads~\cite{Michel2019}, only target inference~\cite{Hadifar2020}. % due to non contiguous access of memory~\cite{Narang2017}. %rn has to be

%Vooturi2020, 



%Additionally, extending unstructured sparse training algorithm to structures typically leads to strong degradation in task performance~\cite{Mostafa2019}  kernel level granularity in DynSparse training~\cite{Mostafa2019}


% Naive extensions of unstructured sparse training algorithms to structure is often only achieved at large task performance loss, e.g

% Developing structured sparse training algorithms is therefore an active field of research, by extending unstructured sparse training algorithms to structure sparsity using structure inducing regularization~\cite{Narang2017, Mummadi2019a}towards , 
% %Increasing the structures of the sparsity pattern through the use of coarse grained sparsity, e.g. on filter, neurons or layers level, ensures a contiguous access of memory, however, often at a task performance cost. 
% There exist ongoing efforts for for  %Reducing the 
% %Structured sparsity patterns are often introduced in order to combine the benefits of sparsity with the performance of dense matrix multiplication. . %~\cite{Zhu2017}
% In particularly, blocksparsity ensures a contiguous access of memory 
% %Fine-tuning objective of large scale language models has been found to be amenable towards sparsity~\cite{Sanh2020}.% paper does not reference blocks but github does  

% While there has been work looking at. Most work on structured pruning relies on the training of a dense network representation augmented by a .
% Adapt architecture using dynamic sparse training towards structured\cite{Yuan2020}
% The dynamic sparsity library used in this work both unstructured and structured sparsity.



%Ramanujan Bipartite Graph Products\cite{Vooturi2020}
% \cite{Hadifar2020} is a conditional sparsity approach, where a block-wise pruned version of the network is used depending on the input. 
% In Ref. {Hadifar2020}, the authors aim at speeding up inference by using conditional sparsity as a form of input-dependent dynamic pruning to conditionally ignore entire blocks.
% In previous work authors have explored block-sparse connectivity
% patterns as ways of combining the benefits of sparsity with the performance of dense matrix multiplication
% on modern hardware. 
% Similarly, grouped convolutions [Xie et al., 2017] and depth-wise separable convolutions [Simonyan
% and Zisserman, 2015] can be interpreted as block-sparse operations. Narang et al. [2017] looked into
% learning block-sparse weight matrices for RNNs. Gray et al. [2017] explore the implementation of
% highly performant CUDA kernels for block-sparse matrix multiplication.
% Structured pruning of language models on fine-tuning~\cite{Wang2021}
% In the original GPU block sparse kernels by Gray~\cite{Gray2017}, the fixed pre-defined block sparsity patterns were chosen to satisfies properties of small world networks. More specifically, in small world networks the graph shows clustering of nodes into communities and a power-law of the  degree distribution. The blocks in the sparsity pattern already guarantee clustering by construction. The power-law in the degree distribution of the underlying sparse graph is proposed to be achieved through Barabasi-Albert, which iteratively and stochastically grows the block sparsity pattern according to degrees of the nodes or distances. 
% However, there are exception as the input dependent blocksparsity in Ref.~\cite{Hadifar2020}, which was shown to outperform a static baseline.
% Topology~\cite{Liu2020} the authors measures to characterise the distance between different sparse graphs. 
%We have found that gradual pruning of blocks of weights often performs competitive with group lasso regularization in agreement with the block pruning versus group lasso experiments in Ref.~\cite{Narang2017}.
% Both static and dynamic sparsity lead to a more computationally efficient sparse network topology with reduced total number of network parameters through the elimination of both edges and nodes in the underlying computation graph.
% As recently pointed out by Yann LeCun at NeurIPS 2019, for sparse computations it would be especially efficient to take advantage of structured sparsity patterns. In fact, irregular sparsity typically breaks the general assumptions of hardware acceleration. However, one can introduce some level of structure, for example in a convolutional layer by pruning entire parameter kernels (and hence the corresponding feature maps), or in a feed-forward layer by pruning parameters corresponding to blocks of input-output connections of a certain size.\par 

%\paragraph{Role of droupout}

% Dropout corresponds to the stochastic elimination of specific inputs or parameters for each batch~\cite{Srivastava2014}. Dropout can therefore be viewed as switching between transient sparsity pattern with every batch. In fact, part of the original motivation for dropout was the ability to take advantage from a sample of different sparsity topologies combined in a single network~\cite{Hinton2012a}. Similarly, an irregular and potentially unstructured static sparsity pattern and its associated irregular network topology also imposes diversity on the computational graph. Despite the sparsity pattern being fixed, we therefore still expect a regularizing effect through the sparsity pattern. 

% Variational dropout~\cite{Kingma2015a} is a generalization of dropout, based on the connection between dropout and Bayesian inference, that allows to learn weight dependent dropout rates~\cite{Molchanov2017}. Variational dropout has been shown to achieve competitive performance on image processing tasks, but has been struggling on neural machine translation~\cite{Gale2019}. \par 
% In Ref.~\cite{Louizos2017a}, the authors impose a sparsity inducing $L_0$ regularization and use a set of stochastic gates, whose parameters are learned in conjunction to the network parameters. While the gates are initialized such as to mimic the stochastic elimination of dropout at initialization, the amount of stochastic elimination is learned and increases during training, leading to a  an increased theoretical FLOPs reduction compared to the theoretical savings from dropout.\par 
